Fault-Tolerant Partial Replication in Large-Scale Database Systems

We investigate a decentralised approach to committing transactions in a replicated database, under partial replication. Previous protocols either re-execute transactions entirely and/or compute a total order of transactions. In contrast, ours applies update values, and orders only conflicting transactions. It results that transactions execute faster, and distributed databases commit in small committees. Both effects contribute to preserve scalability as the number of databases and transactions increase. Our algorithm ensures serializability, and is live and safe in spite of faults.

==> TAGS <==

main.tex,5435
\section { Introduction }102,2481
to thousands of nodes \cite{oceanstore-asplos,muthitacharoen02ivy,DBLP:conf/europar/BuscaPS05}oceanstore-asplos,muthitacharoen02ivy,DBLP:conf/europar/BuscaPS05108,2719
At the cluster level protocols based on group communication primitives \cite{1273036,kemme00dont,1107766}1273036,kemme00dont,1107766111,2872
are the most promising solutions to replicate database systems \cite{1048870}1048870112,2979
Section \ref{sect:model}sect:model133,3652
Section \ref{sect:algorithm}sect:algorithm134,3715
We conclude in Section \ref{sect:end}sect:end135,3768
\section { System model and assumptions }138,3894
\label{sect:model}sect:model139,3936
  Our taxonomy comes from \cite{defago00totally}defago00totally156,4560
  This service is strictly weaker than the classical eventual leader service \leader \cite{leaderRaynal}leaderRaynal201,6561
\subsection { Operations and locks }213,7162
    \label{tab:lock}tab:lock231,7625
Table \ref{tab:lock}tab:lock260,8600
In Table \ref{tab:lock}tab:lock264,8818
\subsection { Transactions }293,9704
\section { The algorithm }312,10529
\label{sect:algorithm}sect:algorithm313,10556
Serializability theory tell us that this relation must be acyclic \cite{syn:db:1467}syn:db:1467317,10682
\subsection { Overview }334,11385
\label{sect:overview}sect:overview335,11410
Section \ref{sect:variants}sect:variants339,11544
\subsection { Initial execution phase }369,12527
\label{sect:init}sect:init370,12567
according to the two-phases locking rule \cite{syn:db:1467}syn:db:1467373,12645
\subsection { Submission phase }389,13125
\label{sect:com}sect:com390,13158
\subsection { Certification phase }406,13652
\label{sect:cert}sect:cert407,13688
$o$ and $o'$ share the lock (see Table \ref{tab:lock}tab:lock448,15217
\subsection { Precedence graph } 457,15444
\label{sect:pgraph}sect:pgraph458,15478
\subsection { Deciding }515,17527
  \caption{\label{alg:decide}alg:decide518,17580
    \If { $T \in \breakCycles{G'}$ } \label{alg:decide:cb}alg:decide:cb531,17924
the literature about this problem is vast \cite{574848}574848552,18750
Algorithm~\ref{alg:decide}alg:decide558,19075
\subsection{ Closure phase }561,19157
  \replicas{\outgoingNeighborsI{T}} (line \ref{alg:lsdb:7}alg:lsdb:7575,19632
  Then $i$ merges $G$ to \Gi (lines \ref{alg:lsdb:8}alg:lsdb:8581,19955
  \caption{\label{alg:lsdb}alg:lsdb607,20676
        \State \commit{T} \label{alg:lsdb:0}alg:lsdb:0621,21072
    \When { \rmdeliver{T} } \label{alg:lsdb:1}alg:lsdb:1627,21181
      \EndFor \label{alg:lsdb:2}alg:lsdb:2630,21360
    \When { $ \exists o \in \pending \land  i = \wleader{\replicas{o}} $}  \label{alg:lsdb:3}alg:lsdb:3633,21407
        \State \tomcast{o} to \replicas{o}  \label{alg:lsdb:4}alg:lsdb:4634,21501
    \WhenFT { $ \tomdeliver{o} $ } \label{alg:lsdb:4b}alg:lsdb:4b638,21583
        \State \setAbortedI{T} \label{alg:lsdb:4c}alg:lsdb:4c644,22021
        \ForAll{ $ o': \precedesI{o'}{o} $ } \label{alg:lsdb:5}alg:lsdb:5647,22143
            \State $ \edges{\Gi} \assign \edges{\Gi} \union \{ (\trans{o'}, T) \} $ \label{alg:lsdb:6}alg:lsdb:6648,22207
      \State \send{\predecessorsI{T}} to \replicas{\outgoingNeighborsI{T}} \label{alg:lsdb:7}alg:lsdb:7651,22339
    \When { \receive{T,G} } \label{alg:lsdb:8}alg:lsdb:8655,22450
            \State \send{\predecessors{T}{\Gi \union G}} to \replicas{\outgoingNeighborsI{T}} \label{alg:lsdb:9}alg:lsdb:9658,22614
    \State $\Gi \assign \Gi \union G$ \label{alg:lsdb:10}alg:lsdb:10661,22756
    } \Comment{Commitment} \label{alg:lsdb:11}alg:lsdb:11676,23072
\subsection { Commitment phase }687,23322
\label{sect:commit}sect:commit688,23355
$i$ commits $T$ as soon as $T$ is executed (line \ref{alg:lsdb:0}alg:lsdb:0691,23431
(line \ref{alg:lsdb:10}alg:lsdb:10695,23603
Algorithm~\ref{alg:lsdb}alg:lsdb705,24035
on a single site \cite{syn:db:1467}syn:db:1467709,24216
\subsection { Initial execution on more than one site } 713,24301
\label{sect:variants}sect:variants714,24358
\subsection { Performance analysis }736,25363
We consider Paxos \cite{Lam06}Lam06738,25401
and $od$ replicas execute line \ref{alg:lsdb:7}alg:lsdb:7749,26008
\section { Concluding remarks } 753,26239
\label{sect:end}sect:end754,26272
\subsection { Related work }756,26290
Gray et al. \cite{233330}233330758,26320
Wiesmann and Schiper confirm practically this result \cite{1048870}1048870762,26536
Fritzke et al. \cite{879303}879303763,26605
Preventive replication \cite{1107766}1107766767,26830
The epidemic algorithm of Holiday et al \cite{holliday02partial}holliday02partial770,26994
scale-up of the system \cite{alonso97partial}alonso97partial777,27322
The DataBase State Machine approach \cite{citeulike:552795}citeulike:552795779,27370
Its extensions \cite{LABOS-CONF-2006-024,sousa01partial}LABOS-CONF-2006-024,sousa01partial781,27496
is a well-known technique \cite{shih90survey}shih90survey785,27683
Recently Haller et al. have proposed to apply it \cite{1099563}1099563786,27730
\subsection { Conclusion } 789,27879
Replication \cite{359563}359563800,28469
Total Order Multicast \cite{defago00totally}defago00totally801,28534
  In \cite{359563}359563804,28594
  In \cite{defago00totally}defago00totally806,28692
\label{lastpage}lastpage814,28998
\renewcommand{\url}\url819,29067
\appendix825,29139

Makefile,1318
FILE=1,0
FINAL=2,10
MAKEFLAGS=4,35
GPSOURCE=7,91
EPSSOURCE=10,124
BIBS=13,158
TEXIN=16,212
DEPS=19,246
GRAPHICSSOURCE=25,362
EPSGRAPHICS=27,405
PDFGRAPHICS=29,453
GNUPLOT=31,491
default:default33,510
${FINAL}.pdf ${FINAL}.ps.gz final:${FINAL}.pdf ${FINAL}.ps.gz final35,530
tags etags:tags etags46,797
TAGS:TAGS48,815
graphics:graphics51,887
epsgraphics:epsgraphics53,922
pdfgraphics:pdfgraphics55,951
dvi:dvi57,980
$(FILE).dvi ${FILE}.aux:$(FILE).dvi ${FILE}.aux59,999
pdf:pdf63,1119
force:force68,1218
${FILE}.bbl:${FILE}.bbl71,1286
clean:clean77,1466
bib:bib80,1488
clean:clean84,1538
spotless:spotless87,1611
ps:ps90,1666
gz ps.gz:gz ps.gz97,1786
print lpr:print lpr99,1811
gv:gv102,1872
$(FILE).dvi:$(FILE).dvi105,1913
%.prn:%.prn107,1947
clean:clean109,2030
%.eps:%.eps112,2052
%.eps:%.eps114,2086
%.eps:%.eps118,2153
%.eps:%.eps120,2189
clean:clean122,2217
%.eps:%.eps125,2248
%.eps:%.eps129,2305
clean:clean131,2336
%.dvi:%.dvi134,2358
%.ps:%.ps139,2507
%.ps.gz:%.ps.gz142,2552
%.pdf:%.pdf144,2582
%.pdf:%.pdf146,2605
clean:clean148,2632
sub1.prn sub2.prn sub3.prn sub4.prn sub5.prn:sub1.prn sub2.prn sub3.prn sub4.prn sub5.prn152,2679
pdffigs.tgz:pdffigs.tgz154,2813
epsfigs.tgz:epsfigs.tgz156,2877
tgz:tgz159,2942

macros.sty,6257
\renewcommand{\labelitemi}\labelitemi2,29
\newcommand{\xor}\xor5,95
\newcommand{\union}\union6,121
\newcommand{\inter}\inter7,147
\newcommand{\bigunion}\bigunion8,173
\newcommand{\biginter}\biginter9,228
\newcommand{\bottom}\bottom10,260
\newcommand{\equaldef}\equaldef11,287
\newcommand{\equivdef}\equivdef12,348
\newcommand{\iftxt}\iftxt13,404
\newcommand{\ifftxt}\ifftxt14,441
\renewcommand{\implies}\implies16,506
\renewcommand{\impliedby}\impliedby17,543
\renewcommand{\iff}\iff19,599
\newcommand{\Henceforth}\Henceforth20,636
\newcommand{\Eventually}\Eventually21,667
\renewcommand{\emptyset}\emptyset22,702
\newcommand{\true}\true23,738
\newcommand{\false}\false24,785
\newcommand{\notimplies}\notimplies25,834
\newcommand{\equals}\equals26,887
\newcommand{\pp}\pp27,924
\renewcommand{\ensuremath}\ensuremath32,1023
\newcommand{\assign}\assign35,1095
\newcommand{\abs}\abs36,1139
\newcommand{\nequals}\nequals37,1179
\newcommand{\braket}\braket38,1234
\newenvironment{preuve}preuve48,1548
\newenvironment{proposition}proposition64,1981
\newcommand{\qed}\qed68,2103
\newenvironment{theorem}theorem72,2189
\newcommand{\sites}\sites91,2611
\newcommand{\leader}\leader92,2649
\newcommand{\wleader}\wleader93,2691
\newcommand{\wleaderSite}\wleaderSite94,2751
\newcommand{\faulty}\faulty96,2821
\newcommand{\correct}\correct97,2879
\newcommand{\hb}\hb100,2957
\newcommand{\cc}\cc101,2981
\newcommand{\emathit}\emathit103,3010
\newcommand{\emathitpar}\emathitpar104,3061
\newcommand{\send}\send108,3162
\newcommand{\receive}\receive109,3214
\newcommand{\receiveSite}\receiveSite110,3272
\newcommand{\rbcast}\rbcast112,3360
\newcommand{\rdeliver}\rdeliver113,3421
\newcommand{\rdeliverSite}\rdeliverSite114,3482
\newcommand{\abcast}\abcast116,3571
\newcommand{\abdeliver}\abdeliver117,3633
\newcommand{\abdeliverSite}\abdeliverSite118,3696
\newcommand{\abdeliverI}\abdeliverI119,3768
\newcommand{\rmcast}\rmcast121,3850
\newcommand{\rmdeliver}\rmdeliver122,3911
\newcommand{\rmdeliverSite}\rmdeliverSite123,3973
\newcommand{\tomcast}\tomcast125,4078
\newcommand{\tomcastSite}\tomcastSite126,4141
\newcommand{\tomdeliver}\tomdeliver127,4213
\newcommand{\tomdeliverSite}\tomdeliverSite128,4277
\newcommand{\tomdeliverI}\tomdeliverI129,4350
\newcommand{\data}\data135,4469
\newcommand{\transactions}\transactions136,4513
\newcommand{\commit}\commit138,4566
\newcommand{\abort}\abort139,4615
\newcommand{\submitted}\submitted141,4663
\newcommand{\committed}\committed142,4718
\newcommand{\aborted}\aborted143,4773
\newcommand{\committedI}\committedI145,4825
\newcommand{\abortedI}\abortedI146,4876
\newcommand{\replicas}\replicas148,4924
\newcommand{\ditem}\ditem149,4977
\newcommand{\isRead}\isRead150,5023
\newcommand{\isWrite}\isWrite151,5072
\newcommand{\order}\order153,5124
\newcommand{\ro}\ro154,5170
\newcommand{\wo}\wo155,5211
\newcommand{\uv}\uv156,5252
\newcommand{\trans}\trans157,5293
\newcommand{\conflict}\conflict158,5340
\newcommand{\initialExecution}\initialExecution161,5405
\newcommand{\releaseIwLocks}\releaseIwLocks162,5483
\newcommand{\forceWriteLock}\forceWriteLock163,5557
\newcommand{\applyUpdates}\applyUpdates164,5631
\newcommand{\holdLock}\holdLock165,5701
\newcommand{\holdIwLocks}\holdIwLocks166,5763
\newcommand{\mvsg}\mvsg169,5857
\newcommand{\versionOrder}\versionOrder170,5905
\newcommand{\ec}\ec173,5974
\newcommand{\ser}\ser174,6002
\newcommand{\si}\si175,6032
\newcommand{\gsi}\gsi176,6060
\newcommand{\pcsi}\pcsi177,6090
\newcommand{\snapshot}\snapshot179,6123
\newcommand{\workflow}\workflow180,6176
\newcommand{\emptyGraph}\emptyGraph186,6297
\newcommand{\pgraphSite}\pgraphSite188,6359
\newcommand{\Gi}\Gi189,6408
\newcommand{\pgraphSiteTime}\pgraphSiteTime190,6454
\newcommand{\Git}\Git191,6510
\newcommand{\vertices}\vertices193,6565
\newcommand{\edges}\edges194,6622
\newcommand{\weight}\weight195,6676
\newcommand{\incomingNeighbors}\incomingNeighbors197,6727
\newcommand{\incomingNeighborsI}\incomingNeighborsI198,6786
\newcommand{\incomingNeighborsIT}\incomingNeighborsIT199,6847
\newcommand{\outgoingNeighbors}\outgoingNeighbors201,6911
\newcommand{\outgoingNeighborsI}\outgoingNeighborsI202,6971
\newcommand{\outgoingNeighborsIT}\outgoingNeighborsIT203,7033
\newcommand{\predecessors}\predecessors205,7098
\newcommand{\predecessorsI}\predecessorsI206,7154
\newcommand{\predecessorsIT}\predecessorsIT207,7208
\newcommand{\successors}\successors209,7265
\newcommand{\successorsI}\successorsI210,7319
\newcommand{\successorsIT}\successorsIT211,7369
\newcommand{\cyclesNat}\cyclesNat213,7422
\newcommand{\cycles}\cycles214,7477
\newcommand{\precedenceGraphs}\precedenceGraphs219,7597
\newcommand{\precedenceGraph}\precedenceGraph221,7654
\newcommand{\isCommitted}\isCommitted223,7722
\newcommand{\isCommittedI}\isCommittedI224,7793
\newcommand{\setCommitted}\setCommitted225,7846
\newcommand{\setCommittedI}\setCommittedI226,7919
\newcommand{\isAborted}\isAborted228,7975
\newcommand{\isAbortedI}\isAbortedI229,8042
\newcommand{\setAborted}\setAborted230,8091
\newcommand{\setAbortedI}\setAbortedI231,8160
\newcommand{\witnesses}\witnesses233,8212
\newcommand{\witnessesI}\witnessesI234,8279
\newcommand{\closed}\closed236,8329
\newcommand{\closedI}\closedI237,8381
\newcommand{\op}\op239,8425
\newcommand{\opg}\opg240,8475
\newcommand{\lsdb}\lsdb245,8613
\newcommand{\Variable}\Variable247,8666
\newcommand{\Variables}\Variables248,8722
\renewcommand{\Return}\Return249,8780
\newcommand{\breakCycles}\breakCycles253,8983
\newcommand{\predecessorsAlg}\predecessorsAlg254,9051
\newcommand{\purge}\purge255,9131
\newcommand{\decide}\decide256,9192
\newcommand{\run}\run262,9300
\newcommand{\precedesRelation}\precedesRelation264,9338
\newcommand{\precedesSite}\precedesSite265,9395
\newcommand{\precedesI}\precedesI266,9470
\newcommand{\precedes}\precedes267,9523
\newcommand{\pending}\pending269,9590
\newcommand{\pendingSite}\pendingSite270,9643
\newcommand{\pendingI}\pendingI271,9708
\newcommand{\limit}\limit273,9747

